Four Years of FAccT: A Reflexive, Mixed-Methods Analysis of Research Contributions, Shortcomings, and Future Prospects

Fairness, Accountability, and Transparency (FAccT) for socio-technical systems has been a thriving area of research in recent years. An ACM conference bearing the same name has been the central venue for scholars in this area to come together, provide peer feedback to one another, and publish their work. This reflexive study aims to shed light on FAccT's activities to date and identify major gaps and opportunities for translating contributions into broader positive impact. To this end, we utilize a mixed-methods research design. On the qualitative front, we develop a protocol for reviewing and coding prior FAccT papers, tracing their distribution of topics, methods, datasets, and disciplinary roots. We also design and administer a questionnaire to reflect the voices of FAccT community members and affiliates on a wide range of topics. On the quantitative front, we use the full text and citation network associated with prior FAccT publications to provide further evidence about topics and values represented in FAccT. We organize the findings from our analysis into four main dimensions: the themes present in FAccT scholarship, the values that underpin the work, the impact of the contributions both within academic circles and beyond, and the practices and informal norms of the community that has formed around FAccT. Finally, our work identifies several suggestions on directions for change, as voiced by community members.

==> section/DEPRECATED_critiques.tex <==
%\section{Voices from the FAccT Community: Criticisms and Suggestions}\label{sec:critiques}

Through a variety of open-ended questions, we found that participants had many opinions about FAccT. The responses indicate that affiliates care about the FAccT community and the directions that FAccT scholarship moves. They also reveal a number of unresolved conflicts and tensions that exist in the community. In this section, we report a coding analysis of participants' responses to our open-ended questions about 
(1) the most important \emph{criticisms} of FAccT scholarship to date;
(2) \emph{suggestions} for addressing them in the near future;
(3) and any other thoughts about FAccT.
Responses covered a wide spectrum of opinions, ranging from broadly positive to highly negative, but the bulk of responses fell somewhere in between--raising significant shortcomings while recommending steps for improvement. 
 
\xhdr{Coding process}
42 (out of 60) participants responded to at least one of the above questions with criticisms and suggestions. Their responses formed the qualitative data at the core of our analysis in this section. We utilize manual coding to organize this data and extract higher order themes from it. The output of our coding process is summarized in Table~\ref{table:defense}.
Following the steps proposed by \citet{tesch2013qualitative}, our coding proceeded as follows: First, we read all responses to get a sense of their overall sentiments.
Second, we went through responses participant by participant. For each individual, we winnowed their responses by summarizing them into higher-level critiques and suggestions.
Third, we clustered similar critiques and suggestions and abbreviated each cluster's topic to form an initial set of codes.
Fourth, we went back to the original responses to ensure that our codes appropriately organizes the data. This exercise led us to adjusting and merging a handful of codes. The third column in Table~\ref{table:defense} demonstrates our final set of codes corresponding to the topic of criticisms. To the extent possible, we mapped suggestions to criticisms.
Finally, based on the object and subject of the critique, we grouped the codes into seven categories--illustrated in the second column of Table~\ref{table:defense}---addressing FAccT as a venue, the culture of the affiliated research community, and the scholarly work published in FAccT. \blcomment{I wonder if we should explain the coding process in Section 5.1 (defining impact) or earlier and simply reference it here? In my coding of FAccT papers I noticed that there are a bunch of papers that using coding practices and simply drop a quick cite rather than explain the process in full.}

\subsection{FAccT as a Venue} \blcomment{should this be ``conference'' to match the table ``applicability''?} 

We categorize the concerns about FAccT as a \textit{venue} into (1) issues regarding FAccT's organization internally and (2) issues regarding FAccT's relationship with other industries, disciplines, and interests.

\xhdr{Peer review quality} Peer review quality was identified as an issue for FAccT based on responses. One respondent noted that the review quality is a particular challenge for FAccT because of the varied discplinary expertise of FAccT affiliates: \qt{By becoming broad and interdisciplinary, it has harmed the review process, and thus the quality of the paper. E.g., legal scholars and humanities scholars are reviewing computer science papers without proper expertise.} The responses corroborate the survey result reported in Section~\ref{subsection:interdisciplinarity}. Luckily, a number of participants who noted the problem of peer review quality suggested solutions; reported in Table~\ref{table:defense}. We categorize these solutions into (1) improving transparency (2) standards, in order to make the quality and selectivity more even and onboard reviewers systematically, and (3) separate tracks/reviews based on STEM, HSA, and non-academic contributions.

\xhdr{Over-curation} One participant stated, \qt{There may be too much "curation" of the accepted papers and tutorials. We should strive to accept all work that is novel, correct and fits the scope of the conference without being too cute about it.} Another stated, \qt{There may be too much "curation" of the accepted papers and tutorials. We should strive to accept all work that is novel, correct and fits the scope of the conference without being too cute about it.} \blcomment{I have trouble defining this. Hoda, could you fill this in?}

\xhdr{Industry influence} A significant portion of responses brought up industry and corporate influence in FAccT's organization, including its executive committee. While we found a variety of critiques related to FAccT's broader relationship to industry (which we discuss later), an emergent theme was the positionality of industry employees in key positions in the conference. One participant stated, \qt{The FAccT community should be more careful in how researchers from big tech industry are assigned key positions in the conference.} Another called for FAccT to \qt{limit corporate researchers' involvement with the EC.}

%One response described why industry influence can have a harmful impact: \qt{It is easy for industry to adopt (or co-opt) some aspects of the work in ways which only minimally help those affected by algorithmic systems, and may even make them worse by giving them a false sense of legitimacy.} A number of responses suggested strategies for confronting this set of issues---these suggestions are listed in Table~\ref{table:defense} and the full set of answers are available in the Appendix \blcomment{Appendix reference}. 

\xhdr{Other organizational concerns} A number of unique suggestions cropped up which we highlight. First, one response characterized the conference organization as \qt{erratic and unpredictable,} \blcomment{will people find this insulting?} especially regarding changes to deadlines and CFPs. Second, a respondent brought up environmental concerns associated with travel: \qt{As a community we should be more thoughtful about the carbon footprint associated with air travel.}

\ 

\xhdr{Relationship to Industry} Now turning away from FAccT's organizational structures and decisions and and focusing on the FAccT conference's relations to other organizations, we start by noting the emergent theme of industry relations, connections, and scholarship. One response succinctly stated: \qt{By and large, FAccT an ethics-washing machine for big tech.} In discussing the role of industry research and its representation in FAccT, respondents acknowledged that this is a complex question. One respondent called for FAccT to \qt{figure out a way to enable industry to meaningfully contribute (there are many good researchers out there, despite the poor dynamics we've read about in the past year).} Others expressed the opposite sentiment: \qt{FAccT scholarship's relationship with industrial research is complex. Some questions are not asked or are difficult to ask within industrial research. There is a political bias.}

\xhdr{Relationship to Public Sector and Government} One response emphasized focusing more on \qt{government and public sector [to] compel people to address more problems in affected communities}.

\xhdr{Other discplinary venues} One emergent critique was a lack of \qt{interplay with `standard' CS conferences}. One participant stated that FAccT \qt{"isolates people who are concerned with values-oriented work from the main body of the technical community."}. Another critique was the idea that the \qt{work gets published without addressing key social scientific expertise.} 

\subsection{FAccT's Internal Culture}

\xhdr{Activisim-oriented vs. scientific agendas} A number of responses criticized the FAccT community \qt{viewing research with a specific ideological prism rather than a scientific prism.} One response described this tension: \qt{There's a real tension in the community between those who see incremental progress as progress and those who believe the only meaningful progress will be revolutionary. I'm not sure how to resolve this, but thus far the community has been expansive enough for both camps. I'm not sure how long that can or will last. Sometimes I worry that work I'm preparing will seem "apologist" to elements of the community since it's not "activist" enough. But I'm also sympathetic to the calls for more activism and supportive of pushing the community in that direction.}


\xhdr{Non-constructive critisism}
\qt{FAccT scholarship is all about [criticism] now ... Do we want to be a community of people that *does* stuff or a community of people that *complains* about stuff?} Another participant stated, \qt{There are 2 polarizing camps - the mathematical, theoretical algorithmic fairness group and the lets-burn-everything-down social aspects group. Reality lies somewhere in the middle and we don't directly address working with actual groups or communities. Everything is a critique from a distance. We must get closer.} %Another respondent identifies the challenge of \qt{how best to meld together people doing very mathematical stuff with those doing very critical theoretic stuff to get the best out of everyone.}

\xhdr{Ingroup-outgroup dynamics}
One respondent states that FAccT is not immune from the cultural effects of \qt{groups and cliques} and that people should \qt{focus less on social media.}

\xhdr{Animosity toward STEM}
One participant stated, \qt{I attended FAccT in-person and found that there was an extreme amount of animosity towards `engineers' and other technical people, which is honestly shocking for a conference about fairness, accountability and transparency. I found myself in several situations where people would speak with true disdain towards engineers, as though this was commonplace and normal.}

\xhdr{Lack of inclusivity}
One response called for \qt{increased outreach (including financial assistance) for participants from minoritised communities and identities.} \blcomment{Is this an organizational critique?}

\xhdr{Misc. (risk for junior researchers, social media)} One emergent theme we highlight is consideration for junior researchers, given the uncertain nature of FAccT as a scholarly community and how young the conference is. Another theme was the impact of social media, which tended to stoke in-group out-group dynamics and non-constructive criticism.

\ 

\xhdr{Collaborations} Responses noted that it is important for FAccT to be interdisciplinary. One stated, \qt{FAccT is one of the best examples of a conference that celebrates multi- and interdisciplinarity.} However, some respondents stated that FAccT actually lacks \qt{truly interdisciplinary collaboration.} A number of responses called for a specific award for collaborative and inter-disciplinary work.

\xhdr{Communications} One respondent pointed out a \qt{lack of integration between FAccT and philosophical community (including ethicists, political philosophers), due to the technical nature of FAccT scholarship.}  Others call for \qt{Engage[ment] with more social sciences and humanities disciplines} and a \qt{greater inclusion of perspectives from other disciplines.}

\xhdr{Contribution and novelty}
One participant stated, \qt{It is not uncommon for individuals to be exposed to a handful of papers, persons, and ideas that are not in their area of expertise, and then think they can produce new scholarship on that basis, because the field encourages `interdisciplinarity.'} Another stated, \qt{It is hard to show novelty of a research contribution to peers from other disciplines. Thus, there is a risk to publish contributions with limited novelty.}

\subsection{FAccT Scholarship}

\xhdr{Lack of practical impact} 
\qt{Compel people to address actual problems with impacted communities.}

\xhdr{Intellectualism / echo-chamber dynamics}
\qt{The FAccT community can be slightly insular and like an echo chamber ... and FAccT scholarship may be less impactful than it could be if this is ignored and communities continue to diverge.}

\xhdr{Solutionism}
One critique was that \qt{the technical papers can be overly solutionist}. Respondents emphasized that \qt{not everything has/needs a computational solution.}
One respondent stated that FAccT scholarship has \qt{a tendency to not fundamentally question certain technologies or discuss in what contexts they're (in)appropriate (e.g. risk assessment instruments in criminal justice, child welfare) - instead a tendency to incrementally improve such technologies.}

\xhdr{Lack of engagement with domain expertise}

\qt{Sometimes work gets published without addressing key social scientific expertise.}
\qt{My work bridges research and production applications, and I sometimes get the sense that folks engaged in research don't understand how little people outside of the FAccT community understand about the scholarship and work. There's a tension between our ideals and meeting people where they are.}

\xhdr{Lack of public- and community engagement}


\xhdr{Lack of diversity and inclusion}
One response called for \qt{Diversity in authors, reviewers, and general participants.} Another called for adding \qt{diversity and inclusion} as a value of import other than fairness, accountability and transparency.

\xhdr{Fairness}
\qt{technical/technocratic approaches to fairness (i.e. many CS definitions) do not sufficiently or offer a very narrow view of more broadly understood conceptions of fairness in law, policy, society; de-biased systems don't necessarily mean they are free from bias}
\qt{The over-emphasis on operationalization / technical definitions of fairness.}

\xhdr{Machine Learning}
\qt{an over-emphasis on machine learning instead of other types of computer-driven technology (in fact, I don't think I've ever read a paper that didn't in some way have to do with ML.}

\xhdr{Western- and U.S.-centric values} An emergent theme was Western- and U.S.-centrism in FAccT's orientation and values. \qt{western orientation of moral and social values.} Another response stated, \qt{The conversation in FAccT often assumes a strong familiarity with a set of values and modes of discourse which are currently highly visible in the US, but much less so in other countries, especially non-Western countries. I urge the community to consider what can be done to make researchers who are not fluent in this specific type of discourse feel welcome and able to participate in the community.}

\xhdr{Risk of ``fair-washing''}
One respondent stated that FAccT \qt{gets used to "fair-wash" existing practices.} Another called FAccT an \qt{ethics-washing organization}

\xhdr{Ontology}
\qt{FAccT has not yet settled key ontological questions about the field, leading to incoherent use of key terms, such as "AI" and "algorithm".}

\xhdr{Lack of critical evaluation of mathematical assumptions}
One response noted \qt{an over focus on technical results without careful considerations for the mathematical assumptions and constraints use}.

\xhdr{Discouraging mathematical contributions}
One response stated, \qt{many researchers feel unwelcome in FAccT and that they need to be walking on eggshells rather than engage in scientific and mathematical discourse, and makes students scared to present.} Another response stated, \qt{My understanding is that FAccT currently features publications from two pretty different communities: a more social science/philosophy group and a more computer science/math group. Some friction between these groups is probably a feature, not a bug, of a conference like this. But back when I worked on fairness stuff, it made me less likely to submit technical material to FAccT, because I looked at the social science/philosophy papers and thought a lot of them weren't very good.}

\subsection{Potential Remedies}

\xhdr{Improving review}
\begin{itemize}
    \item \xhdr{Separate Tracks and Reviewing Pools by Expertise}
One respondent cautioned against separate tracks: \qt{I think FAccT should strive to be a space that transcends specific disciplinary standards and traditions rather than perpetuating them. We should make more effort to have reviewers from more disciplines rather than creating silos where papers are reviewed only by members of their own disciplines. Otherwise FAccT will just be perpetuating the disciplinary conservatism that already exists within each discipline.}

    \item \xhdr{Transparency and Standards}
    Standards
    Expose expertise
    Education/onboarding process
    
    \item \xhdr{Constructive Criticism Phase} \qt{I would encourage developing a more thorough constructive criticism approach. Peer review tends to focus on the quality of the scholarship. And then the conference shows off the work, inviting questions during the presentations.  I think that once papers are ready, there should be another stage which is constructive criticism where people are invited to challenge the assumptions/values/agendas of the work, to push researchers towards equity and justice more actively.}
\end{itemize}

\xhdr{Industry Influence}

\qt{Implement stricter funding disclosures for submitted manuscripts, limit corporate researchers' involvement with the EC, diversify the EC, promote CRAFT, adjust bylaws to make clear FAccT is not an auditing organization.}

Other participants suggested that industry researchers \textit{should} play a role, and that FAccT just needs to clarify what a productive role should be: \qt{include more social, political, and design researchers + figure out a way to enable industry to meaningfully contribute (there are many good researchers out there, despite the poor dynamics we've read about in the past year)}

\xhdr{}

\xhdr{}
